Modelling ion acceleration and transport in corotating interaction regions: the mass-to-charge ratio dependence of the particle spectrum

We investigate the role of perpendicular diffusion in shaping energetic ion spectrum in corotating interaction regions (CIRs), focusing on its mass-to-charge ($A/Q$) dependence. We simulate a synthetic CIR using the EUropean Heliospheric FORcasting Information Asset (EUHFORIA) and model the subsequent ion acceleration and transport by solving the focused transport equation incorporating both parallel and perpendicular diffusion. Our results reveal distinct differences in ion spectra between scenarios with and without perpendicular diffusion. In the absence of perpendicular diffusion, ion spectra near CIRs show a strong $(A/Q)^{\epsilon}$ dependence with $\epsilon$ depending on the turbulence spectral index, agreeing with theoretical predictions. In contrast, the incorporation of perpendicular diffusion, characterized by a weak $A/Q$ dependence, leading to similar spectra for different ion species. This qualitatively agrees with observations of energetic particles in CIRs.

==> abbrev.tex <==
\usepackage{xspace}
\newcommand{\aj}{AJ\xspace}
\newcommand{\apj}{ApJ}
\newcommand{\apjl}{ApJ\xspace}
\newcommand{\apjlett}{ApJ\xspace}
\newcommand{\apjs}{ApJS\xspace}
\newcommand{\apjsupp}{ApJS\xspace}
\newcommand{\aap}{A\&A}
\newcommand{\astap}{A\&A\xspace}
\newcommand{\araa}{ARA\&A\xspace}
\newcommand{\aapr}{A\&A Rev.\xspace}
\newcommand{\aaps}{A\&AS\xspace}
\newcommand{\mnras}{MNRAS\xspace}
\newcommand{\pasp}{PASP\xspace}
\newcommand{\apss}{Ap\&SS\xspace}
\newcommand{\pasj}{PASJ\xspace}
\newcommand{\nat}{Nature\xspace}
\newcommand{\sci}{Science\xspace}
\newcommand{\skytel}{S\&T\xspace}
\newcommand{\memras}{MmRAS\xspace}
\newcommand{\qjras}{QJRAS\xspace}
\newcommand{\jrasc}{JRASC\xspace}
\newcommand{\baas}{BAAS\xspace}
\newcommand{\iauc}{IAU Circ.\xspace}
\newcommand{\iaucirc}{IAU Circ.\xspace}
\newcommand{\aplett}{Astrophys. Lett.\xspace}
\newcommand{\apspr}{Astrophys. Space Phys. Res.\xspace}
\newcommand{\bain}{Bull. Astron. Inst. Netherlands\xspace}
\newcommand{\fcp}{Fund. Cosmic Phys.\xspace}
\newcommand{\aipconf}{AIP Conf. Proc.\xspace}
\newcommand{\aspconf}{ASP Conf. Ser.\xspace}
\newcommand{\asslconf}{Ap\&SSL Conf. Ser.\xspace}
\newcommand{\procspie}{Proc. SPIE\xspace}
\newcommand{\maps}{MAPS\xspace}
\newcommand{\planss}{Planet. Space Sci.\xspace}
\newcommand{\ssr}{Space Sci. Rev.}
\newcommand{\ao}{Appl. Opt.\xspace}
\newcommand{\applopt}{Appl. Opt.\xspace}
\newcommand{\solphys}{Sol. Phys.}
\newcommand{\pra}{Phys. Rev. A\xspace}
\newcommand{\prb}{Phys. Rev. B\xspace}
\newcommand{\prc}{Phys. Rev. C\xspace}
\newcommand{\prd}{Phys. Rev. D\xspace}
\newcommand{\pre}{Phys. Rev. E\xspace}
\newcommand{\prl}{Phys. Rev. Lett.\xspace}
\newcommand{\rmp}{Rev. Mod. Phys.\xspace}
\newcommand{\grl}{Geophys. Res. Lett.}
\newcommand{\jgr}{J. Geophys. Res.\xspace}
\newcommand{\adv}{Adv. Space Res.\xspace}
\newcommand{\icrc}{ICRC}
\newcommand{\jswsc}{J. Space Weather Space Clim.}
\newcommand{\jcp}{	J. Chem. Phys.}
\newcommand{\jpp}{	J. Plasma Phys.}
